Modality Gap-Driven Subspace Alignment Training Paradigm For Multimodal Large Language Models

Despite the success of multimodal contrastive learning in aligning visual and linguistic representations, a persistent geometric anomaly, the Modality Gap, remains: embeddings of distinct modalities expressing identical semantics occupy systematically offset regions. Prior approaches to bridge this gap are largely limited by oversimplified isotropic assumptions, hindering their application in large-scale scenarios. In this paper, we address these limitations by precisely characterizing the geometric shape of the modality gap and leveraging it for efficient model scaling. First, we propose the Fixed-frame Modality Gap Theory, which decomposes the modality gap within a frozen reference frame into stable biases and anisotropic residuals. Guided by this precise modeling, we introduce ReAlign, a training-free modality alignment strategy. Utilizing statistics from massive unpaired data, ReAlign aligns text representation into the image representation distribution via a three-step process comprising Anchor, Trace, and Centroid Alignment, thereby explicitly rectifying geometric misalignment. Building on ReAlign, we propose ReVision, a scalable training paradigm for Multimodal Large Language Models~(MLLMs). ReVision integrates ReAlign into the pretraining stage, enabling the model to learn the distribution of visual representations from unpaired text before visual instruction tuning, without the need for large-scale, high-quality image-text pairs. Our framework demonstrates that statistically aligned unpaired data can effectively substitute for expensive image-text pairs, offering a robust path for the efficient scaling of MLLMs.

==> Fig/Fig1_intro.tex <==
\begin{figure}[t]
    \centering
    % -----------------------------------------------------------
    % Custom Colors
    % -----------------------------------------------------------
    \definecolor{sybcblue}{HTML}{004488}  % Visual
    \definecolor{brickred}{HTML}{BB5566}  % Textual
    \definecolor{softgray}{HTML}{666666}  % Geometry
    % -----------------------------------------------------------

    \resizebox{0.85\columnwidth}{!}{%
    \begin{tikzpicture}[
        >={Latex[length=3mm, width=2mm]}, 
        font=\sffamily,
        % Styles
        target shape/.style={ellipse, draw=sybcblue, thick, fill=sybcblue!10, align=center, inner sep=2pt},
        source shape/.style={ellipse, draw=brickred, thick, dashed, fill=brickred!10, align=center, inner sep=2pt},
        axis/.style={->, draw=softgray, thick},
        label bg/.style={fill=white, fill opacity=0.85, text opacity=1, rounded corners=2pt, inner sep=1pt},
        halo/.style={preaction={draw=white, -, line width=3.5pt}} 
    ]
    
    % =========================================================
    % 1. Reference Frame
    % =========================================================
    \begin{scope}[local bounding box=geometryFrame]
        
        % --- Subspace U (Floor) ---
        \begin{scope}[transform canvas={xslant=0.5, yscale=0.4}]
            \draw[step=1cm, softgray!15, thin] (-2.5,-2.5) grid (2.5,2.5);
            \draw[draw=softgray!40, thick] (-2.5,-2.5) rectangle (2.5,2.5);
            \node[softgray, font=\bfseries\small, anchor=south east] at (2.5,-2.5) {Subspace $U$};
        \end{scope}
        
        % --- V Axis (Vertical) ---
        \draw[axis, ultra thick] (0,0) -- (0, 2.3);
        \node[anchor=west, font=\bfseries, xshift=2pt] at (0, 2.3) {$V$};
        \node[anchor=west, softgray, font=\scriptsize, xshift=2pt, yshift=-8pt] at (0, 2.3) {};
        
        % Principal axis guide
        \draw[axis, dashed, thin] (0,0) -- (2.2, 0.6); 
        \node[softgray, font=\tiny, rotate=10, anchor=west] at (2.2, 0.6) {};

        % =========================================================
        % 2. Distributions
        % =========================================================

        % --- Text Distribution (Top Left) ---
        % 旋转了 -5 度
        \node[source shape, minimum width=2.2cm, minimum height=1.2cm, rotate=-5] (txtDist) at (-1.7, 1.8) {};
        
        % --- Image Distribution (Bottom Right) ---
        % 旋转了 5 度
        \node[target shape, minimum width=2.6cm, minimum height=1.0cm, rotate=5] (imgDist) at (1.8, 0.5) {};

        % =========================================================
        % 3. Arrow & Labels
        % =========================================================

        % --- Stable Bias Arrow ---
        \draw[->, softgray, line width=1.5pt, halo] (txtDist.center) -- 
            node[midway, sloped, font=\footnotesize\bfseries, fill=white, inner sep=1pt] {Stable Bias}
            (imgDist.center);

        % --- Centers & Type Labels ---
        \fill[brickred] (txtDist.center) circle (1.5pt); 
        \node[brickred, font=\small\bfseries, above=0.1cm] at (txtDist.north) {Textual Representation};

        \fill[sybcblue] (imgDist.center) circle (1.5pt);
        \node[sybcblue, font=\small\bfseries, below=0.15cm] at (imgDist.south) {Visual Representation};

        % --- Anisotropy Arrows ---
        
        % 红色箭头 (Anisotropic)
        % 修改处：改为使用极坐标确保精确倾斜 -5 度，与标签和椭圆平行
        \draw[<->, brickred, thin] ($(txtDist.center)+(175:0.6)$) -- ($(txtDist.center)+(-5:0.6)$);
        % 标签位置在下方(south)，角度为-5，保持不变
        \node[brickred, font=\tiny, rotate=-5, inner sep=0.5pt] at ($(txtDist.south)+(0, 0.3)$) {Anisotropic};

        % 蓝色箭头 (Residuals)
        % 使用极坐标确保精确倾斜 5 度
        \draw[<->, sybcblue, thin] ($(imgDist.center)+(185:0.7)$) -- ($(imgDist.center)+(5:0.7)$); 
        % 标签位置在下方(south)，角度为5
        \node[sybcblue, font=\tiny, rotate=5, inner sep=0.5pt] at ($(imgDist.south)+(0, 0.25)$) {Residuals};

    \end{scope}
    \end{tikzpicture}
    }
    \vspace{12pt}
    \caption{Geometric decomposition of the modality gap. We characterize the intrinsic shape of the modality gap within a frozen reference frame. Unlike prior isotropic assumptions, we reveal that the gap consists of a systematic Stable Bias and Anisotropic Residuals. This precise modeling serves as the theoretical foundation for our statistical alignment strategy.}
    \label{fig:modality_gap}
    \vskip -0.1in
\end{figure}
